Low-Latency Video Semantic Segmentation

Recent years have seen remarkable progress in semantic segmentation. Yet, it remains a challenging task to apply segmentation techniques to video-based applications. Specifically, the high throughput of video streams, the sheer cost of running fully convolutional networks, together with the low-latency requirements in many real-world applications, e.g. autonomous driving, present a significant challenge to the design of the video segmentation framework. To tackle this combined challenge, we develop a framework for video semantic segmentation, which incorporates two novel components: (1) a feature propagation module that adaptively fuses features over time via spatially variant convolution, thus reducing the cost of per-frame computation; and (2) an adaptive scheduler that dynamically allocate computation based on accuracy prediction. Both components work together to ensure low latency while maintaining high segmentation quality. On both Cityscapes and CamVid, the proposed framework obtained competitive performance compared to the state of the art, while substantially reducing the latency, from 360 ms to 119 ms.

==> camvid_show.tex <==
\begin{figure*}
\centering
%\setlength{\fboxsep}{1cm}
  %\fbox{\includegraphics[totalheight=2in]{pend.eps}}

\begin{tabular}{@{\hspace{0mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c}
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/1201.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/1202.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/1203.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/1204.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/1205.png}\\
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/key_label_1201_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/key_label_1202_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/key_label_1203_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/key_label_1204_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1200/key_label_1205_color.png}\\


\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/1301.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/1302.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/1303.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/1304.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/1305.png}\\
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/key_label_1301_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/key_label_1302_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/key_label_1303_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/key_label_1304_color.png} &
\includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1300/key_label_1305_color.png}\\


% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/1401.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/1402.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/1403.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/1404.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/1405.png}\\
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/key_label_1401_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/key_label_1402_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/key_label_1403_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/key_label_1404_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/camvid_data-master/1400/key_label_1405_color.png}\\


\end{tabular}
\caption{Visual Results for CamVid Dataset}
\label{fig:camvid}
\end{figure*}


==> cityshow.tex <==

\begin{figure*}
\centering
%\setlength{\fboxsep}{1cm}
  %\fbox{\includegraphics[totalheight=2in]{pend.eps}}

\begin{tabular}{@{\hspace{0mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c}
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/000000_015371_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/000000_015372_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/000000_015373_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/000000_015374_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/000000_015375_leftImg8bit.png}\\
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/key_label_15371_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/key_label_15372_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/key_label_15373_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/key_label_15374_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/015389/key_label_15375_color.png}\\


\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/000000_017210_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/000000_017211_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/000000_017212_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/000000_017213_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/000000_017214_leftImg8bit.png}\\
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/key_label_17210_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/key_label_17211_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/key_label_17212_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/key_label_17213_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/017228/key_label_17214_color.png}\\


\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/000001_037687_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/000001_037688_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/000001_037689_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/000001_037690_leftImg8bit.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/000001_037691_leftImg8bit.png}\\
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/key_label_37687_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/key_label_37688_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/key_label_37689_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/key_label_37690_color.png} &
\includegraphics[width=0.19\linewidth]{figures/paper_data2/037705/key_label_37691_color.png}\\

%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/000001_055288_leftImg8bit.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/000001_055289_leftImg8bit.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/000001_055290_leftImg8bit.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/000001_055291_leftImg8bit.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/000001_055292_leftImg8bit.png}\\
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/key_label_55288_color.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/key_label_55289_color.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/key_label_55290_color.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/key_label_55291_color.png} &
%\includegraphics[width=0.19\linewidth]{figures/paper_data2/055306/key_label_55292_color.png}\\

% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/000001_060527_leftImg8bit.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/000001_060528_leftImg8bit.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/000001_060529_leftImg8bit.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/000001_060530_leftImg8bit.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/000001_060531_leftImg8bit.png}\\
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/key_label_60527_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/key_label_60528_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/key_label_60529_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/key_label_60530_color.png} &
% \includegraphics[width=0.19\linewidth]{figures/paper_data2/060545/key_label_60531_color.png}\\

\end{tabular}
\caption{Visual Results for Cityscapes Dataset}
\label{res:cityscapes}
\end{figure*}


==> model.tex <==
% !TEX root = vseg_main.tex

\section{Model Formulation}
\label{sec:model}
%Our  goal in this work is to reduce not only the overall cost but also the maximum latency. 
Our proposed framework is based on the insight that the content of  adjacent frames over a video move smothly and there representatoins of deep network change slowly corespondingly as showed in~\cite{shelhamer2016clockwork}. So processing video frame by frame is not needed, and the keyframe-based method is proposed to reduce the overall cost in work of Clockwork network~\cite{shelhamer2016clockwork} and
Deep Feature Flow (DFF)~\cite{zhu2016deep}. Naturally, we should ask the question: when is frame selected as the keyframe and can we reduce the overall cost and maintain a low-latency at the same time?

To answer the question, we design a scheduling module to determine the keyframe adaptively and an adaptive feature propagation module to reduce the overall cost. The maximum latency can be reduced by a schedule scheme and improved further by parameters and computation share with both modules and the per-frame prediction network. The time steps of our low-latency pipeline is viewed in Fig~\ref{model_details}. Only at time step $T_1$ both low part and high part of basic network are forwarded to obtain the label and cache the high-level feature, which cause the maxinum latency of the whole video. At next time step, the low part of basic network(figure~\ref{model_details}(a)) is forwarded to provide the low level feature for schedule module(figure~\ref{model_details}(b)) and feature progagation module(figure~\ref{model_details}(c)). Whether high part of basic network is forwarded or not depends on the output of adaptive schedule. When the adaptive schedule outputs $no$, the high part of basic network is not excuted and save the computation cost as showed in $T_2,T_3$. When it ouputs $yes$, the high part of basic network is excuted underlying and the pipeline is not blocked as showed in $T_4$. At the same time, although the frame is labeled as keyframe, the feature propagation module still propagate the high level feature from previous keyframe and its output is just cached to be propagated at the next time steps as showed in $T_5$, thus reducing the maxinum latency.

In what follows, we will start to introduce schedule scheme of our low-latency pipeline to illustrate how the componets work togather to achieve the goal in a global perspective, then explain  the mechanism of all components of schedule scheme: the basic network structure, the adaptive feature propagation module and adaptive schedule module respectively. 

%In this paper, we propose a novel video segmentation framework which contains an adaptive feature propagation module and an adaptive scheduling module.
%The former is primarily for propagating features across frames via a spatially variant scheme,
%while the latter is to learn a better key-frame schedule.
%Both modules share parameters and computation with the per-frame prediction network, thus only incurring marginal computational burden. The entire pipeline can reduce latency significantly, while still maintaining high segmentation accuracy.

%In particular, our framework cache the low-level and high-level features of the key frames to provide history information. When a new frame comes, low-level feature is extracted by the basic network, and its corresponding high-level representation is directly updated by our adaptive propagation module with small latency. It follows by an adaptive schedule module to predict whether current frame should be a new key-frame. If it is labeled as a key-frame, it will go through the rest of the basic network to update the key-frame feature. Both the adaptive propagation and adaptive schedule module contain marginal cost, so the overall cost can be reduced by skipping the heavy computation of high-level feature from the basic network.
%\jpshi{May need a figure}
%\dahua{Please summarize the overall pipeline here and describe how different modules work
%together in a bird's eye view. For example, when a new frame comes,
%what it would do. How it determines whether it is a key frame or not, how it processes
%a key frame and a non-key frame. This roadmap is important to prevent the audience from
%getting lost.}

%In what follows, we will start with a description of our basic network structure, then explain the adaptive feature propagation module and adaptive schedule module respectively. Finally, we will discuss a scheme specifically designed to achieve low latency.

%Overview your method
%Our model aims to obtains video semantic with low computational cost and low delay. As work  based on resnet in PSP\ref{} and deeplab\ref{}, semantic segmentation frame by frame shows good performance, but it suffer from low comutational cost and high delay. When resnet is applied to video, the key is how to reuse the feature of resnet by taking advantage of the consistency information of video frames. We first disgin a featue  propagation model to transfer feature of resnet from key frame to current frame effectively.
%The feature propagation model is much smaller than resnet, which  reduces the amount of computation and delay effectively. It's also very critical to adaptly schedule key frame for video frames vary greatly in different time periods. So We further designed a shedule predict model to scheduling key frame dynamically. The overview of our model show as \ref{model_details}. We first indroduce the resnet baseline, then describe the feature propagation model and schedule prediction and finally present the low latency schedule scheme.

\begin{figure*}[t]
\centering
%\flushright
 %\includegraphics[width = 0.8\linewidth]{framework}%
 \includegraphics[width = 1.0\linewidth]{pipeline}%
 \caption[model compare]{Time steps of our low-latency pipeline. Note some inputs of purple block at each time step is omited, the whole structure of which can be viewed in (c). At time step $T_{1}$, all componets of basic network (a) are ran to obtain label and the output of high part of network($S_{h}$) is cached. At time step $T_{i}(i>1)$, whether $S_h$ is forwarded or not depends on the output of adaptive schedule (b). When $S_h$ is scheduled (showed as $T_4$), its output is cached and will be propagated to future frame at next time steps(showed as $T_5$), otherwise it's not excuted (showed as $T_2,T_3$).} \label{model_details}
\end{figure*}




\subsection{Low Latency Schedule Scheme}
Latency is very important for real-world applications
while it has not received much attention from previous work.
Given  the basic network module(detailed in subsection\ref{subsec:basic_network}), the feature propagation module(detailed in subsection\ref{subsec:feature_prop}) and the adaptive schedule prediction module(detailed in subsection\ref{subsec:schedule_pred}),
we combine them into a late key-frame replacement schedule scheme to reduce latency.



%\begin{figure}[t]
%\centering
%%\flushright
% \includegraphics[width=\linewidth]{schedule_scheme.pdf}%
%
% \caption[schedule scheme]{a: late propagation schedule; b: immediate propagation schedule.}\label{schedule_scheme}
%
%\end{figure}


%\paragraph{Late propagation schedule}
%\dahua{The following statement has grammatical issues, please fix:
%
The core of our designed scheduler is that, even if the key frame is detected in frame $t$, we still get temporal high level feature $\hat{\mathcal{F}}_h^t$ from propagation as showed as $T_4$ in Fig.~\ref{model_details}.
So the overall latency is reduced by not blocking by feature forward in heavy high-level network $S_h$.
The accurate high level feature $\mathcal{F}_h^t$ is updated afterwards as key-frame reference for future frame propagation.
%Non-key frame will continue without further computation through the heavy $S_h$ subnetwork. But key frame will go through the rest of the ResNet blocks $S_h$ to replace with more reliable $\mathcal{F}_h$ for future frame propagation.
Although the low latency propagation will hurt performance to some extent, our adaptive feature propagation and adaptive schedule will compensate the system as a whole. The overall algorithm is illustrated in Algorithm~\ref{alg}. To summarize, such late key-frame replacement schedule pipeline is very effective for real applications.



% $t$ while $\mathcal{F}_h^t $ is still propagated from last key frame, for the excute of $S_h$ is very time-consuming and the system should not block to wait the result of $S_h$. For the next frames the $\mathcal{F}_h^{t+i} $ can be propagated from frame $t$ or frame $k$, which depends whether the $\mathcal{F}_h^t $ is ready. We call it late propagation schedul is because the $\mathcal{F}_h^t $ is still propagated from last key frame when a new key frame is detected. Obviously this schedule scheme can maitains the lowest latency, while it may sacrifice certain accuracy for the $\mathcal{F}_h^{t+i} $ may not be propagated from frame $t$ when $i$ is less $L$， where $L$ is determined by ratio of time of $S_h$ and $S_l$.

%\paragraph{Immediate propagation schedule}
%n this schedule scheme, one first split the $S_h$ to two sub-phases $S_{h^d}$ and $S_{h^u}$. When the key frame is detected in frame $t$,$S_{h^d}$ will be excuted immediately. So in the next frame $t+1$, the feature $\mathcal{F}_h^{t+1} $ is immediately propagated from $\mathcal{F}_{h^d}^t $. Then in the next frames the feature  $\mathcal{F}_h^{t+i+1} $ can be propagated from frame $t$, which may cause certain delay for $F_{h^u}^t$ may be  not accessed. This schedule scheme may get good performance for it propagated the nearest frame feature, but increase certain latency for it need to wait the result of  $S_{h^u}$ to some extent.


\begin{algorithm}[t]
\caption{Late Key-Frame Feature Replacement Scheduling}\label{alg}
\begin{algorithmic}[1]
\State Forward $S_l$, $S_h$ and cache key frame feature $\mathcal{F}_l^k$ and $\mathcal{F}_h^k$ at $t=1$ and initilize it as key frame
\For {time $t > 1$} 
\State $\mathcal{F}_l^t \gets$ Forward network $S_l$
\State $\hat{\mathcal{F}}_h^t$ $\gets$ adaptive propagation module
\State Predict final result based on $\hat{\mathcal{F}}_h^t$
\State \textit{is\_keyframe} $\gets$ adaptive schedule module
\If {\textit{is\_keyframe}}
\State $\mathcal{F}_h^t \gets$ Forward $S_h$
\State Label frame $t$ as key frame
\State Cache $\mathcal{F}_l^t$ and $\mathcal{F}_h^t$ as key frame feature
\EndIf
\EndFor
\end{algorithmic}
\end{algorithm}


%In practice, We choice the late propagation stragety as our schedule scheme, for it do not need add any compoonets and can maintain the lowest latency.






\subsection{Basic Network}
\label{subsec:basic_network}
%Introduce the basic network, each part of the ResNet is used in later section as what function....
We use ResNet101~\cite{he2015deep} as our baseline model given its superior performance on semantic segmentation. We divide the network into two parts: $S_l$ and $S_h$, as shown in Figure~\ref{model_details} (a) in separate dash boxes.
Specifically, the lower part of the network, denoted as $S_l$, contains layers from the input to the layer \texttt{conv4\_3}. The higher part of the network, denoted as $S_h$, contains the layers afterwards. %In particular, the feature map $\mathcal{F}_l$ produced by the lower part $S_l$ are connected via a shortcut to the higher-layer features $\mathcal{F}_h$, in order to provide more localization information.
%Moreover, $\mathcal{F}_l$ can be further used in the adaptive propagation module.

The lower part of the network works as a feature extractor for key frame prediction, adaptive propagation, and as well adaptive scheduling. Generally the computation cost for $S_l$ is much smaller than that of $S_h$.
%Thus this intermediate feature $\mathcal{F_l}$ by the \texttt{conv3\_3} can be regarded as information exchange platform between history frames and current frames.
In practice, we can set a different intermediate layer as the separating point or even increase the number of separating layers based on the trade-off between speed and performance.

During video processing, the lower part of the network $S_l$ is executed at each frame, and its output feature map $\mathcal{F}_l$ is utilized as input to the adaptive propagation module. The adaptive propagation module predicts spatially variant propagation weights based on $\mathcal{F}_l$, which is further utilized to control the
propagation of the higher-layer features $\mathcal{F}_h$ from the key-frame to current frame.
Then the adaptive scheduler determines whether current frame should become the next key-frame based on $\mathcal{F}_l$. The higher layer of the network $S_h$ is only executed when it is labeled as a key frame.

%When resnet101 is applied to segment semanticly image, it can be represented as $I -> S_l -> F_l -> S_h -> F_h -> l$, where $I$ is input iamge, the  $F_l$ and $F_h$  are the feature extracted by $S_l$ and  by $S_h$ respectively and $l$ represent the semantic label. The computational cost of $S_l$ is generally much samller than $S_h$. As figure \ref{model_details} a,  both $S_l$ and $S_h$ should execute when resnet runs on video frame by frame. We will extend it by feature propagation model, which almost just run $S_l$ and sparsely run $S_h$ when scheduled by schedule prediction module.

\subsection{Adaptive Feature Propagation}
\label{subsec:feature_prop}
%Explain the feature propagation by figures, illustration, and equations.

Our feature propagation module as shown in Fig.\ref{propagation} is aimed to propagate
$\mathcal{F}_h^k$, the high-level features of the key frame, to $\mathcal{F}_h^c$,
that of the current frame. As the illustraction in Fig.\ref{propagation} , the high level feature $F_{h}^c(i,j)$ is similar to its neighbors in $\mathcal{F}_h^k$ as shown in red block in Fig.\ref{propagation} . We express this similarity by weighting the feature within its neighbors in $\mathcal{F}_h^k$ into $\mathcal{F}_h^c$. Further, as shown different red blocks in Fig.\ref{propagation} , the feature $F_{h}^c(i,j)$ in different location has its own adaptive weights. We use a small net to predict the adaptive weights which recieve the intermediate lower layer feature $\mathcal{F}_l$ as the input.
%based on both the low-level features $\mathcal{F}_l^k$ in the key frame and $\mathcal{F}_l^c$ in the current frame.
%
We use the intermediate lower layer feature $\mathcal{F}_l$ as the input for weight propagation for three reasons. First, it contains more semantic information than the raw input. Second, the shared computation on $S_l$ reduces the overall computation compared to a complete optical flow net. Moreover, we learn a weighted propagation, instead of a strict point-to-point propagation as optical flow, which introduces more freedom to our system.


\begin{figure}[t]
\centering
%\flushright
 \includegraphics[width = 1\linewidth]{figures/adaptive_propagation}%

 \caption{ Adaptive feature propagation. The high level feature $F_{h}^c(i,j)$ is similar to its neighbors in $\mathcal{F}_h^k$, and different location has different similarity as different red blocks shown. When $\mathcal{F}_h^k$ is propagated to $F_{h}^c$ it should have its own adaptive combination weights, denoted as the heatmap in feature map which is learned
 by a adaptive propagation module.}\label{propagation}
\end{figure}

%Our weight propagation module, denoted as green block in Fig.~\ref{model_details} (c), contains 2 convolution layers together with non-linear transform batch normalization and ReLU layer. Output of the weight propagation module is normalized by a softmax layer to represent probability, which is a 25 dimension feature, representing the 5x5 weights to fusing the high level feature $\mathcal{F}_h$. \jpshi{Yule, please correct me with details about the model design. Including how many convolution layers, etc.} Therefore, we can get a different weight combination for different location with current observation on low level features.

Our weight propagation module is detailed as in Fig.~\ref{model_details} (c). The high level feature $F_{h}^c(i,j)$ at each location in current frame is obtained by applying the sum of weights in its neighour window of key frame with $H \times H$ size.  Each location has its own propagation weights and the weights are shared cross different channels. The propagation pattern at each location for high level feature is predicted by a fully convolution net. It contains $3$ convolutional layers together with interlaced ReLU layers. The output of the weight propagation module at each location is converted into probability values via a softmax layer,
which is a map of size $H \times H$, representing the $H \times H$ weights to fuse the high-level feature $\mathcal{F}_h$. The example is shown as Fig\ref{propagation} , the heatmap represents the weights and  the brightness value represents the corresponding weight magnitude. We encode the $H \times H$ dimensional feature to channels to adapt to the structure of FCN. In our experiments, we set $H = 9$.
%The details of weight propagation module can be show as tabel\ref{weight_prop_net}.
In this way, we can get a different weight combination for different location based on the current observations of low-level features.

%\begin{table}[htbp]
%\caption{weight propagation net}\label{weight_prop_net}
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{c|c|c|c}
%\hline
%name & type & stride &\#output \\
%\hline
%conv1 & 3x3 conv & 1 &	512 \\
%\hline
%conv2 & 3x3 conv &	1 &	1024 \\
%\hline
%conv3 & 1x1 conv &	1 &	1024 \\
%\hline
%weight\_prop & 1x1 conv & 1 & HxH	 \\
%\hline
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\end{table}

After we got the propagation weights, the adaptive propagation can then be formulated as a spatially variant convolution operator. Specifically, given $\mathcal{F}_h$, the high-level feature map for the key frame, the high-level features for the current frame can be computed as
%As figure \ref{model_details} b, our model runs $S_l$ on every video frames with low computational cost. So for time $t$, we extract feature map $F_{l\_t}$ of frame $I_t$ using $S_l$ and $F_{l\_kt}$ of frame $I_{kt}$ is cached in histoy frame which don't need to be computated in time $t$. The feature map $F_{h\_kt}$ extracted by $S_h$ in time $kt$ is also cached, and our goal is to predict the feature map $F_{h\_t}=f(F_{h\_kt},F_{l\_kt},F_{l\_t})$. Our hypothesis is  that feature vector of location $(i,j)$ in $F_{h\_t}$ of current frame $t$ is similar to it neighbor vector in $F_{h\_kt}$ of history frame $kt$. We represent the neighbor as $(i+m,j+n)$ where $m \in [-l,l] $ and $n \in [-l,l]$, and $l$ is the size of neighbor window. We use weight $W$ to catch the similarity between $F_{h\_t}(i,j)$ and its neighbor $F_{h\_kt}(i+m,j+n)$ of frame $kt$, which can be formalized as below:
\begin{equation}
F_{h}^c(l,i,j) = W_{ij} \cdot \mathcal{F}_{h}^k(l,i, j)
%F_{h}^c(i,j) = \sum_{m=1}^{m=H}\sum_{n=1}^{n=H}W_{ij}(m,n) \cdot \mathcal{F}_{h}^k(i+m, j+n)
\end{equation}
where $W_{ij}$ is the output of the weighted propagation module at location $(i, j)$ and shared cross different channel $l$.
% $\mathcal{F}_{h}^k(i, j)$ is the high-level feature value for the key frame at $(i, j)$; $\mathcal{F}_{h}^c(i, j)$ is that of the current frame.


%Our model also use neighbor window to catch the context information, the bigger the window size is and the better accuracy it'll be, but it caused to high computational cost and also may be overfit on the dataset. A good choice is to fellow the method of dilation convulotion, we also use hole to extend the receptive field and do not increase any computation cost.


The entire propagation works as a spatially variant depth-wise convolution, to apply different weight to different location and each channel shares weights. It is easy for back propagation, and can be trained end-to-end with other modules. Compared to Clockwork Network~\cite{shelhamer2016clockwork}, which directly replaces history features and fuses via subsequent convolution layers, it is more flexible and powerful due to the spatial variability.
Compared to Deep Feature Flow~\cite{zhu2016deep}, it shares the low-level computation, and provides a weighted propagation than point-to-point propagation, which is more robust in feature space.

%In practice, both the high level feature from weighted propagation module and low level feature from current frame  are concat together for final prediction to increase robustness.
To increase robustness when scene changes frequently, in addition to the propagated high level feature $\mathcal{F}_h^c$,
% we also fuse the output of $\mathcal{F}_l^c$ by a convolution layer and concatenation for further prediction as in Clockwork Net.
we also fuse the output of $\mathcal{F}_l^c$ as in Clockwork Net. Instead of simple concatenation as Clockwork Net, we first apply a AdaptNet to $\mathcal{F}_l^c$, then concatenate the $\mathcal{F}_h^c$, and finally use the fuse module to output the label. The AdaptNet is critial. The low level feature $\mathcal{F}_l^c$ is not suitable to predict semantic label directly and can be further learned by AdaptNet. What's more important, when combined with progapated hight level feature $\mathcal{F}_h^c$ it can learn the complementary information which can't caught by weight propagation due to sudden move. The details of AdaptNet and fuse module follows the section \ref{sec:exper}
%\jpshi{??} The fuse just contains an adaptive layer while promoting the stability of the model greatly.
%Our experiments show the fusing feature increase performance and stability greatly, which
%The effectiveness of this scheme as shown in our experiments indicates that
%the high-level features propagated from history and the low-level features from the current frame have a strong complementary relationship.
%\jpshi{The figure might be changed.}
%We impelement the $g(F_{l\_kt},F_{l\_t})$ using fully convolution network, so the $W$ have the same spatial height and width as $F_h$. The the length of vector $W(i,j)$ is $(2l+1)*(2l+1)$, and we encode it to channels of output of convolution layer.
%The gradient of $\frac{\partial{F_{h\_t}}}{\partial{W}}$ is easy obtained, so the feature propagaton model can be end-to-end trained.

%\subsection{Propagated and Current Feature  Fuse Module}
%The propagated feature from feature propagation module hold of temporal information, which can be complemented by information of current frame. As figure\ref{model_comparation}(c), we pass the feature map $F_{l\_t}$ by a adapted network to $F_{h_t}$.

\subsection{Adaptive Schedule Prediction}
\label{subsec:schedule_pred}
As illustraction of Fig.\ref{schedule}, a natural video segmentation system should arrange more computation resources to difficult regions or with large temporal change frames, and reduce computation when the video sequence is stable. Although many previous works discussed this issue, none of them actually provided an elegant mechanism to achieve this. Till now, what dominate the practice are still simple fixed-rate schedulers or those based on thresholds of feature map variance.

The key to achieve the adaptive scheduling is a suitable loss to assist learning. We treat this as predicting the accuracy of current frame label based on the low-level feature observations. The accuracy is defined to be the fraction of pixels at which both key-frame and current labels are the same. Intuitively, if the final accuracy is high, it should provide confident patterns even in low level feature.
In our design, such prediction is accomplished by a small network with a few convolution layers.

\begin{figure}[t]
\centering
%\flushright
 \includegraphics[width = 1\linewidth]{figures/adaptive_schedule}%

 \caption{ Adaptive schedule. The labels propagated from key frame have different accuracy among sequences,
 which are shown as the blue dot in the top.
 So it is natural that the frame which varies large from previous frames
 should be denoted as key frame and needs more computation.}\label{schedule}
\end{figure}

We treat the label predicted by a pretrained model as an auxiliary label $l$. By analyizing the relation between $ \mathcal{F}_l$ and lable $l$, we run the pretrained baseline network for each video sequence on both Cityscapes and Camvid dataset, to get the low level feature $ \mathcal{F}_l$ and output semantic label $l$, then compute $\vert \mathcal{F}_l^k - \mathcal{F}_l^t \vert $ and $acc(l^k,l^t)$. We all found that when $\vert \mathcal{F}_l^k - \mathcal{F}_l^t \vert $ is bigger, the value of $acc(l^k,l^t)$ is smaller, which implies that the differences among feature maps $\mathcal{F}_l^k$ have a strong relationship with label stability. During the video sequence, the feature difference is strongly related to the accuracy difference. It can also be validated by the two consecutive frames , which has low feature difference and high accuracy difference.

In particular, the adaptive schedule module takes the difference of $\mathcal{F}_l$ as the input, and after three convolutional layers with 128 channels and a fully connected layers, it regress the accuracy of current frame with full key frame inference. An illustration of this adaptive schedule prediction module is shown in Figure~\ref{model_details} (b).
% The details of adaptive schedule module can be show as tabel\ref{adapt_schedule_net}.
%The label is pre-processed by a pretrained model, and used to finetune the adaptive schedule module.  % Some of the representative examples are shown in Fig.~\ref{}. \jpshi{Please add some result illustration for adaptive schedule module.}
At inference time, when the prediction for the adaptive schedule module is lower than a threshold, we label it as a key-frame. The thershold is based on the curve of key-frame update ratio and mIou as descripted in section\ref{exp_adaptive_schedule}. We choose the point that attain the best balance between the update ratio and mIOU on validation set, by looking at the curve of update ratio vs. mIOU. Our experiment validate that the threshold of the predicted accuracy is more robust than the threshold of feature difference.
%\jpshi{Show reason either by examples or by illustrations. }

%\begin{table}[htbp]
%\caption{adapt schedule net}\label{adapt_schedule_net}
%\begin{center}
%\begin{small}
%\begin{sc}
%\begin{tabular}{c|c|c|c}
%\hline
%name & type & stride &\#output \\
%\hline
%conv1 & 3x3 conv & 1 &	512 \\
%\hline
%conv2 & 3x3 conv &	2 &	256 \\
%\hline
%conv3 & 3x3 conv &	3 &	256 \\
%\hline
%fc1 & 1x1 fc & 1 & 1024	 \\
%\hline
%fc2 & 1x1 fc & 1 & 1	 \\
%\hline
%\end{tabular}
%\end{sc}
%\end{small}
%\end{center}
%\end{table}




%a learnable schedule prediction module is to design a penalty loss.
%There are two way to design such loss. One is  embedding it to a end-to-end system $l=f(F_hkt(I_t,I_{t-1},...,),g(F_{l\_kt,F_{\_t}})),$. So we can use ture label to construct loss function, but we need carefully design the end-to-end system, which is leaved as feature work.

%Another way to do this is to tell wheather a pair frames varies greatly. Some work [] using Euclidean loss threshold to decide it. Here we use predicted label of output of resnet to estimate the semantic difference. We calculate the acc of key frame label and current frame label predicted by resnet, then we using a sub-network to predict the $acc$. For resnet has good performance, its predicted label can be accurate enough to represent the ture difference of frame pairs. We futher discretize $acc$ using $a_l$ and $a_h$. We transform the regression problem into a classification problem。

% \begin{equation}\label{math:vm}
%\frac{\partial h_i}{\partial v_m} = \begin{cases}
%1,~~~~~~~~~ acc < a_l \\
%255,~~~~a_l <= acc < a_h \\
%0,acc >= a_h
%\end{cases}
%\end{equation}



